Data-driven Modeling of Granular Chains with Modern Koopman Theory

Externally driven dense packings of particles can exhibit nonlinear wave phenomena that are not described by effective medium theory or linearized approximate models. Such nontrivial wave responses can be exploited to design sound-focusing/scrambling devices, acoustic filters, and analog computational units. At high amplitude vibrations or low confinement pressures, the effect of nonlinear particle contacts becomes increasingly noticeable, and the interplay of nonlinearity, disorder, and discreteness in the system gives rise to remarkable properties, particularly useful in designing structures with exotic properties. In this paper, we build upon the data-driven methods in dynamical system analysis and show that the Koopman spectral theory can be applied to granular crystals, enabling their phase space analysis beyond the linearizable regime and without recourse to any approximations considered in the previous works. We show that a deep neural network can map the dynamics to a latent space where the essential nonlinearity of the granular system unfolds into a high-dimensional linear space. As a proof of concept, we use data from numerical simulations of a two-particle system and evaluate the accuracy of the trajectory predictions under various initial conditions. By incorporating data from experimental measurements, our proposed framework can directly capture the underlying dynamics without imposing any assumptions about the physics model. Spectral analysis of the trained surrogate system can help bridge the gap between the simulation results and the physical realization of granular crystals and facilitate the inverse design of materials with desired behaviors.

==> sections/extension.tex <==
\subsection{Methods}
\label{sec:extensionMethods}
Koopman theory can be extended to nonautonomous systems with state $x$ and input $u$, where the dynamics is written as $x_{t+1}=F(x_t, u_t)$. In this case \cref{eq:koopman} becomes:
\begin{equation}
    g(x_{t+1}, u_{t+1}) = K g(x_t, u_t) 
\end{equation}

Assuming a set of eigenfunctions $\varphi$ and eigenvalues $\lambda$, \cref{eq:deepkoopman} becomes:
\begin{equation}
    K \varphi(x_t, u_t) = \varphi(x_{t+1}, u_{t+1}) = \lambda \varphi(x_t, u_t)
\end{equation}

Koopman operator can be defined on an extended state $\Bar{x}:=[x, u]$, with two separate embedding functions ($\varphi(x, u) = [\varphi_x(x, u), \varphi_u(x, u)]$) to make this framework equivalent to the unforced (autonomous) one discussed in the previous section. It's common to assume that the $\varphi_x(x, u)=\varphi_x(x)$ and in the case of the input without control, we can write $\varphi_u(x, u)=u$. Therefore, the above equation can be written as \cite{Shi.Meng2022}:

\begin{equation}
    \varphi_x(x_{t+1}) = K_{xx} \varphi_x(x_t) + K_{xu} u_t  
\end{equation}

This framework can be incorporated in a linear control scheme for the control of nonlinear systems \cite{Shi.Meng2022}. Here, we utilize this framework for analyzing the effect of excitation amplitude on the dynamical regimes of the granular crystals.

\subsection{Implementation Details}
\label{sec:extensionDetails}
The experiments in the previous section considered a system without any inputs. As noted in \cref{sec:dataDriven}, with slight modifications, Koopman analysis can be extended to nonautonomous systems. With this setup, we are able to obtain the modes of the system's forced response and analyze the effect of excitation amplitude and oscillation frequency in the granular crystals. To this end, we considered a three-particle system with fixed boundaries (\cref{tab:KPC_sim}). Here, the leftmost particle is displaced sinusoidally with a specific amplitude and frequency. This system is equivalent to a driven two-particle system, so the displacement and velocity of the first particle are defined as the input ($u$), and the displacement and velocity of the next two particles will be the state of the system ($x$) (see the notation described previously in \cref{sec:modelingUnforced}).
\begin{table}[h]
\caption{Deep Koopman Network Parameters with Control.}
\vskip -0.1in
\label{tab:KPC_params}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|ccc}
\toprule
    \bfseries Parameter & \bfseries Encoder/Decoder & \bfseries Koopman Network \\
\midrule
    Input Size & $ny=4, nu=2$ & $30$\\
    Hidden Layer & $5 \times [200]$ & \textit{None}\\
    Output Size & $30$ & $30$ \\
    Nonlinearity &  \textit{ELU} &  \textit{None}\\ %Exponential Linear Unit
    Bias & \textit{True} & \textit{False} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

To produce the training dataset, we simulate the system starting from equilibrium positions (initial velocities are zero), and move the first particle on a sinusoidal trajectory with random amplitudes and frequencies sampled uniformly from a predefined range of values. We used the same methods as the previous section to record the trajectories from the numerical simulations, and build the dataset. The network structure and training parameters are provided in \cref{tab:KPC_params} and \cref{tab:KPC_train}, respectively.
\begin{table}[h]
\caption{Simulation Setup for Koopman Analysis with Control.}
\vskip -0.1in
\label{tab:KPC_sim}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|c}
\toprule
    %\bfseries Parameter & \bfseries Value \\
%\midrule
    Simulation Time ($T$) & $1e3$ \\
    Time Step ($\Delta t$) & $5e-3$ \\
    Sampling Rate & no sampling \\ %$400$ \\
    Damping ($B, B_{pp}, B_{pw}$) & $0$ \\
    Stiffness Ratio & $2.3$ \\
    Particle Mass ($m$) & $1$ \\
    Particle Diameter ($\sigma_0$) & $0.1$ \\
    Particle Contacts & \textit{Hertzian} \\
    Packing Fraction ($\phi$) & $1e-1$ \\
    Relaxation Time ($FIRE$) & $1e6$ \\
    Oscillation Amplitude ($A$) & $\in [1e-4, 1e-2]$ \\
    Oscillation Frequency ($f$) & $\in [1, 15]$ \\
    Initial Displacement ($x_0$) & $0$ \\
    Initial Velocity ($v_0$) & $0$ \\
    Number of Trajectories & $1000$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
\begin{table}[h]
\caption{Training Setup for Koopman Analysis with Control.}
\vskip -0.1in
\label{tab:KPC_train}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{c|c}
\toprule
    \bfseries Parameter & \bfseries Value \\
\midrule
    Training Set & $450$ samples \\
    Validation Set & $450$ samples \\
    Test Set & $100$ samples \\
    Prediction Window ($P$) & $200$ steps \\
    Optimizer & \textit{Adam} \\
    Learning Rate & \textit{1e-4} \\
    Epochs & $2e4$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\subsection{Results}
\label{sec:extensionResults}
The loss function is the same as in the previous section (see \cref{eq:koopmanloss}). \cref{fig:dkc_loss} shows the training and validation loss during the training.
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/loss.png}
\caption{\label{fig:dkc_loss}
\textbf{Training and validation loss for the deep Koopman network with control.} The loss function is defined in \cref{eq:koopmanloss}. The network is trained on the displacement and velocity trajectories from a numerically simulated two-particle system that is excited with sinusoidal vibrations with random amplitudes and oscillations.
}
\end{figure}

After training the network, we derived the Koopman mode decomposition including eigenvalues, eigenfunctions, and dynamic modes. The Koopman eigenvalues ($\lambda$) are shown in the complex plane in \cref{fig:dkc_eigenDom} with the colors indicating the value of $c_i$, which quantifies the dominance of each mode in the observed data. 
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenvalues_dominance.png}
\caption{\label{fig:dkc_eigenDom}
\textbf{Koopman eigenvalues for the sinusoidally driven two-particle system.} The eigenvalues determine the frequency of the Koopman modes ($Im(\lambda)$) and their decay/growth rate ($Re(\lambda)$). The blue outline shows the unit circle, and the color of each mode indicates its dominance ($\parallel c_i \parallel$). 
}
\end{figure}

\cref{fig:dkc_eigenRate} shows each mode's decay/growth rate with the frequencies on the horizontal axis. The top six nonzero dominant modes (excluding the complex conjugates) are shown in \cref{fig:dkc_modes}. 
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenvalues_rate.png}
\vskip -0.15in
\caption{\label{fig:dkc_eigenRate}
\textbf{Growth/decay rate of the Koopman modes for the sinusoidally driven two-particle system.} The color indicates the dominance of the modes ($\parallel c_i \parallel$) corresponding to \cref{fig:dkc_eigenDom}. The horizontal axis is the frequency of the mode ($\omega=\log(\lambda)/\Delta t$).
}
\vskip -0.1in
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/modes_new.png}
\vskip -0.15in
\caption{\label{fig:dkc_modes}
\textbf{The temporal structure of the top six nonzero dominant Koopman modes for the two-particle system with control.} In each panel, the blue graph shows the complex mode and the real and imaginary parts of the mode are projected onto each face of the 3D plot.
}
\vskip -0.1in
\end{figure}

To evaluate the network's performance, we selected five sample trajectories from the test set and assigned the initial particle positions and velocities along with the input signal ($u$) to the encoder network. Using the trained Koopman network, we can predict the particle positions and velocities in the subsequent time steps and compare them to the reference trajectory obtained from the numerical simulation. \cref{fig:dkc_preds} presents the reference and predicted trajectories for these five test samples. We also calculated the \textit{Root Mean Squared Error (RMSE)} of each case using \cref{eq:RMSE} and reported the values in \cref{tab:KPC_rmse}.
\begin{table}[h]
\caption{Prediction Error for Sample Trajectories.}
\vskip -0.1in
\label{tab:KPC_rmse}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cc}
\toprule
    \bfseries Sample & \bfseries RMSE \\
\midrule
    1 & $1.385e-02$ \\
    2 & $2.002e-02$ \\
    3 & $1.837e-02$ \\
    4 & $1.414e-03$ \\
    5 & $5.827e-04$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/predictions_new.png}
\caption{\label{fig:dkc_preds}
\textbf{Evaluation of the deep Koopman network with five sample trajectories.} Each row shows a sample from the test set with the input parameters (frequency and amplitude of vibration) indicated above the panel. The plots show the input velocity and displacement (\textbf{left}), and particles' positions and velocities (\textbf{right}). Solid lines in the panels on the right show the true trajectories obtained from the numerical simulations, and the dashed lines represent the network predictions.
}
\vskip -0.3in
\end{figure}
As mentioned, Koopman eigenfunctions map the dynamics into the intrinsic coordinates ($y=\varphi(x)$). However, unlike a Fourier transform, the eigenvalues and eigenfunctions are spatially varying in the mapped linear coordinates, and they can show the properties of the original system. %for a nonlinear oscillator system, they should have radial symmetry.
The superposition of these modes results in the global dynamics of the system.

To visualize the global dynamics of the system, we produced $900$ input sinusoidal waves with amplitudes in $[1e-4, 1e-2]$ and frequencies in $[1, 15]$. The real and imaginary components of the eigenfunction are evaluated for each case and presented in \cref{fig:dkc_eigenfuncReal} and \cref{fig:dkc_eigenfuncImg}. These plots show the spatial structure of the intrinsic coordinates in the latent space.
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenfunctions_real.png}
\caption{\label{fig:dkc_eigenfuncReal}
\textbf{The real component of the Koopman eigenfunctions for the two-particle system with control.} Each panel corresponds to one of the Koopman modes extracted from the trained network. The axes in each panel represent the amplitude and frequency of the input vibrations. The color indicates the contribution of each mode to the system's dynamics for each amplitude-frequency pair.
}
\end{figure}
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenfunctions_img.png}
\caption{\label{fig:dkc_eigenfuncImg}
\textbf{The imaginary component of the Koopman eigenfunctions for the two-particle system with control.} Each panel corresponds to one of the Koopman modes extracted from the trained network. The axes in each panel represent the amplitude and frequency of the input vibrations. The color indicates the contribution of each mode to the system's dynamics for each amplitude-frequency pair.
}
\vskip -0.2in
\end{figure}

We also plotted the particle trajectories in the Koopman intrinsic coordinates as they are projected into the linear latent space. These spatial modes can capture regions with fluctuations, slow and fast dynamics that are present in each trajectory. \cref{fig:dkc_eigenfuncTime} shows the time evolution of the eigenfunctions for various input oscillations. 
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenfunctions_trajs.png}
\vskip -0.1in
\caption{\label{fig:dkc_eigenfuncTime}
\textbf{\boldmath Sample Trajectories of the intrinsic coordinates in time ($\varphi(X(t))$). \unboldmath} The amplitude and frequency of the input are indicated on top of each panel. Each panel corresponds to one initial condition. The color indicates the magnitude of the eigenfunction plotted in time.
}
\vskip -0.1in
\end{figure}

To compare granular systems with different particle configurations of soft and staff particles, we trained the deep Koopman network with data from each configuration and obtained the Koopman mode decomposition (see \cref{fig:dkc_eigenvaluesComp}).
\begin{figure}[h!]
\centering
\includegraphics[width=1.0\columnwidth]{figures/deepkoopman/DKC/eigenvalues_compare.png}
\caption{\label{fig:dkc_eigenvaluesComp}
\textbf{Comparison of the Koopman modes in four distinct particle configurations with a sinusoidal input.} The light/dark grey indicates the soft/stiff particles. For each configuration, the Koopman modes are plotted in the complex plane, where the color of each mode quantifies its dominance ($c_i$).
}
\end{figure}
